PFDepth: Heterogeneous Pinhole-Fisheye Joint Depth Estimation via Distortion-aware Gaussian-Splatted Volumetric Fusion

In this paper, we present the first pinhole-fisheye framework for heterogeneous multi-view depth estimation, PFDepth. Our key insight is to exploit the complementary characteristics of pinhole and fisheye imagery (undistorted vs. distorted, small vs. large FOV, far vs. near field) for joint optimization. PFDepth employs a unified architecture capable of processing arbitrary combinations of pinhole and fisheye cameras with varied intrinsics and extrinsics. Within PFDepth, we first explicitly lift 2D features from each heterogeneous view into a canonical 3D volumetric space. Then, a core module termed Heterogeneous Spatial Fusion is designed to process and fuse distortion-aware volumetric features across overlapping and non-overlapping regions. Additionally, we subtly reformulate the conventional voxel fusion into a novel 3D Gaussian representation, in which learnable latent Gaussian spheres dynamically adapt to local image textures for finer 3D aggregation. Finally, fused volume features are rendered into multi-view depth maps. Through extensive experiments, we demonstrate that PFDepth sets a state-of-the-art performance on KITTI-360 and RealHet datasets over current mainstream depth networks. To the best of our knowledge, this is the first systematic study of heterogeneous pinhole-fisheye depth estimation, offering both technical novelty and valuable empirical insights.

==> tbl/tb4_ablation_for_component.tex <==
\begin{tabular}{c @{}cc ccc c c @{}c @{}c  c @{}c @{}c}
\toprule

\multicolumn{1}{c}{\multirow{2}{*}{Exp.}} &
\multicolumn{2}{c}{Front View} &
\multicolumn{3}{c}{Left View} &
\multicolumn{1}{c}{\multirow{2}{*}{\IdeaOne{}}} &
\multicolumn{3}{c}{Fisheye Performance} &
\multicolumn{3}{c}{Pinhole Performance}
\\
&
\multicolumn{1}{c}{HSF} &
\multicolumn{1}{c}{3DGS} &
\multicolumn{1}{c}{Dpat_v2} &
\multicolumn{1}{c}{CVT} &
\multicolumn{1}{c}{use_skips} &
&
AbsRel↓ &
$\delta_1$↑  & &
AbsRel↓ &
$\delta_1$↑  &

\\

\midrule      

(a) &\cmark &  &  &  & &
\xmark & 7.1 & & 0.277 & - & & -\\

(b) & &\cmark & &  & &
\xmark & - & & - & 7.6 & & 0.582 \\ 


(c) & \cmark & \cmark & &  & &
\cmark & 6.5 (↓0.6) & & 0.229(↓4.8 cm) & 6.7 (↓0.9) & & 0.504(↓7.8cm)  \\ 

\midrule

(d) & & & \cmark  &  & &
\xmark & 5.9 & & 0.193 & - & & -\\

(e) & & & & \cmark & \cmark &
\xmark & - &  & - & 6.4 & & 0.387 \\  

(f) & & & \cmark & \cmark  & \cmark &
\cmark & 5.6 & & 0.161 & 6.1 & & 0.278 \\ 

\bottomrule

\end{tabular}%
